Towards Fully-Automated Materials Discovery via Large-Scale Synthesis Dataset and Expert-Level LLM-as-a-Judge

Materials synthesis is vital for innovations such as energy storage, catalysis, electronics, and biomedical devices. Yet, the process relies heavily on empirical, trial-and-error methods guided by expert intuition. Our work aims to support the materials science community by providing a practical, data-driven resource. We have curated a comprehensive dataset of 17K expert-verified synthesis recipes from open-access literature, which forms the basis of our newly developed benchmark, AlchemyBench. AlchemyBench offers an end-to-end framework that supports research in large language models applied to synthesis prediction. It encompasses key tasks, including raw materials and equipment prediction, synthesis procedure generation, and characterization outcome forecasting. We propose an LLM-as-a-Judge framework that leverages large language models for automated evaluation, demonstrating strong statistical agreement with expert assessments. Overall, our contributions offer a supportive foundation for exploring the capabilities of LLMs in predicting and guiding materials synthesis, ultimately paving the way for more efficient experimental design and accelerated innovation in materials science.

==> old-0213/03_dataset.tex <==
\section{Data Collection and Preparation}
\label{sec:data_collection}

This section details our data collection pipeline, from document retrieval to extracting key synthesis information. We focus on how a large corpus of materials science literature is curated, classified, and annotated with recipes essential for downstream benchmarking tasks.

\subsection{Literature Retrieval and Filtering}
We began by compiling a list of 50 keywords that broadly represent research in materials science, ranging from specific compounds (e.g., ``perovskite,'' ``metal--organic framework'') to broader application domains (e.g., ``battery electrode,'' ``catalysis material''). These keywords were used to query the Semantic Scholar API~\cite{semanticscholar2023}. We restricted the collection of articles that include publicly available PDF files to comply with legal and ethical guidelines for text mining. This process yielded a dataset of 28,685 PDF documents spanning various journals and conferences. 

\subsection{PDF Conversion and Document Categorization}


\begin{figure*}[!ht]
    \begin{subfigure}{.55\textwidth}
        \centering
        \includegraphics[width=\linewidth]{image/data/element_freq_heatmap.png}
        \caption{The distribution of elements in the target material shown in the periodic table}
        \label{fig:data-element-distribution}
    \end{subfigure}
    \begin{subfigure}{.43\textwidth}
        \centering
        \includegraphics[width=\linewidth]{image/data/top10process.png}
        \caption{Distribution of categorized manufacturing methods}
        \label{fig:data-process-distribution}
    \end{subfigure}
    \caption{Data Distribution}
    \label{fig:main-data-distribution}
\end{figure*}


After retrieving the PDFs, we converted each file to Markdown format using the \texttt{PyMuPDFLLM}~\cite{pymupdf4llm2024}. 
The resulting Markdown files preserve paragraph structures and metadata while remaining flexible for downstream tasks (e.g., classification, named entity recognition).
Using the processed Markdown files, we employed GPT-4o~\cite{achiam2023gpt} for an automated categorization step, labeling each article according to:

\begin{itemize}
    \item \textbf{Presence of a synthesis recipe:} Whether the text explicitly provides a detailed experimental procedure.
    \item \textbf{Primary material(s):} The main material name, chemical formula, and class studied (e.g., inorganic oxides, polymers).
    \item \textbf{Process or synthesis route:} The dominant experimental methods (e.g., hydrothermal, solution-based, vapor deposition).
    \item \textbf{Application domain:} The intended use-case (e.g., battery, catalysis, biomedical).
\end{itemize}

Based on these annotations, we identified 17,667 articles (\(\sim62\%\) of the corpus) containing explicit synthesis ``recipes'', making them highly relevant for tasks involving the prediction or generation of experimental protocols.

\subsection{Recipe Extraction}
\label{sec:recipe_extraction}

\subsubsection{Key Information Segmentation}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{image/data/example.png}
    \caption{An actual example of extracted recipe.}
    \label{fig:data-example}
\end{figure*}

For each of the 17,667 articles confirmed to include a synthesis recipe, we extracted five critical components, denoted as \textbf{X}, \(\mathbf{Y_M}\), \(\mathbf{Y_E}\), \(\mathbf{Y_P}\), and \(\mathbf{Y_C}\). These components capture the end-to-end workflow of materials synthesis:

\begin{enumerate}
    \item \textbf{X: Target Material, Synthesis Method, and Application Domain}
    
    A concise summary describing:
    \begin{itemize}
        \item \textit{What is being synthesized?} (e.g., Ni-rich layered oxides)
        \item \textit{Which process is used?} (e.g., solvothermal, sol-gel)
        \item \textit{What is the main application?} (e.g., electrode for lithium-ion batteries)
    \end{itemize}
    
    \item \(\mathbf{Y_M}\): \textbf{Raw Materials}
    
    A list of raw materials (e.g., reagents, solvents) and any quantitative details (e.g., molar ratios, concentrations, masses).
    
    \item \(\mathbf{Y_E}\): \textbf{Synthesis Equipment}
    
    A catalog of apparatus (e.g., furnace, autoclave, spin coater) essential for the synthesis steps.
    
    \item \(\mathbf{Y_P}\): \textbf{Synthesis Procedure}
    
    A step-by-step protocol detailing how the reagents are combined and processed (e.g., reaction times, temperatures, pH, stirring speeds).
    
    \item \(\mathbf{Y_C}\): \textbf{Characterization Methods and Results}
    
    Techniques (e.g., X-ray diffraction, electron microscopy) and outcomes (e.g., crystal structure, particle size, electrochemical performance) used to evaluate the synthesized material.
\end{enumerate}

\subsubsection{LLM-Driven Parsing and Annotation}
The extraction of these elements from each Markdown file was again performed via GPT-4o. We minimized human labor in large-scale annotation by carefully prompting the model to identify and extract relevant text blocks.
Detailed prompts are described in Appendix~\ref{sec:appendix_annotation}.

\subsection{Data Verification and Quality Assessment}
To ensure the accuracy of our automatically extracted recipes, we manually verified sampled recipes by eight domain experts, at least a master's student majoring in materials science. These experts evaluated:

\begin{itemize}
    \item \textbf{Completeness:} Did the extracted text capture the full scope of the reported recipe (\textbf{X}, \(\mathbf{Y_M}\), \(\mathbf{Y_E}\), \(\mathbf{Y_P}\), and \(\mathbf{Y_C}\))?
    \item \textbf{Correctness:} Were critical details like temperature values or reagent amounts accurately extracted?
    \item \textbf{Coherence:} Did the extracted recipe retain coherence and avoid contradictory information?
\end{itemize}

\input{table/data/human_verification}
Preliminary reviews indicate that the \emph{majority} of extracted data is highly accurate, especially for articles with well-structured experimental sections. 

Completeness was assessed with relatively high agreement, indicating that key synthesis details were well captured. While its score was slightly lower than correctness and coherence due to occasional omissions of finer experimental details, such as precise molar ratios or characterization settings, the extracted recipes still provide a strong foundation for understanding synthesis procedures. In contrast, correctness and coherence, despite receiving high scores, showed greater variability among evaluators. Differences in how minor inconsistencies—such as variations in equipment names or missing characterization details—were weighted contributed to this variation. Some evaluators viewed these as negligible, while others applied stricter criteria, highlighting the need for clearer annotation guidelines. Overall, these results suggest that the extraction process is already highly effective and can be further refined to enhance the level of detail captured.

% {\color{red}Comprehensive metrics on precision and recall will be added once the manual verification is complete}% 
% Insert final statistics later.

With the dataset prepared and validated, we now focus on how these recipes are used to define a comprehensive benchmark. In the following section (Section~\ref{sec:benchmark}), we introduce the benchmark that evaluates NLP models on end-to-end materials synthesis prediction, ranging from precursor and equipment inference to procedure generation and characterization outcome forecasting.

\subsection{comparison with Existing Datasets}
A direct comparison with prior dataset is necessary to highlight the advantages of the Open Materials Guide (OMG) dataset.

==> old-0213/03_dataset_v2.tex <==

\section{Data Collection and Preparation}
\label{sec:data_collection}
\ref{sec:data}

\subsection{Motivation: Why is this necessary?}
% 여기에 table + citation 추가해야함.
Despite the growing interest in applying NLP techniques to materials science, no standardized benchmark exists for evaluating synthesis modeling approaches. Existing datasets such as ~\cite{wang2022dataset} and ~\cite{kononova2019text} primarily focus on isolated aspects of synthesis, such as reaction conditions or precursor selection, without offering a structured framework for holistic evaluation. Furthermore, many of these datasets lack validation methods, making it difficult to assess their reliability for real-world applications.

% table 만들어야함
Table???
% ~\ref{tab:dataset_comparison} 
compares OMG with prior datasets, highlighting its key advantages. Unlike previous work, OMG provides a comprehensive, high-quality dataset covering all essential synthesis stages, including raw materials, equipment, procedures, and characterization methods. Additionally, it introduces structured evaluation criteria and expert-verified validation techniques, ensuring both data reliability and benchmark consistency.


\subsection{Collection and Extraction}
We collected synthesis procedures from a large corpus of materials science literature to construct the dataset. We retrieved 28,685 open-access articles using the Semantic Scholar API~\cite{semanticscholar2023}, filtering them based on 50 keywords relevance to ensure they contained experimental synthesis details. Domain experts suggested these keywords to collect diverse literature in materials science.

This section details our data collection pipeline, from document retrieval to extracting key synthesis information. We focus on how a large corpus of materials science literature is curated, classified, and annotated with recipes essential for downstream benchmarking tasks.

\paragraph{PDF Processing and Structure Extraction}
Extracted PDFs were converted into structured Markdown format using \texttt{PyMuPDFLLM}~\cite{pymupdf4llm2024}. This step preserved paragraph structures, section headers, and inline metadata while eliminating non-relevant content such as references and appendices. Given the journals' highly varied formatting styles, we applied rule-based heuristics to segment the documents into meaningful units.

\paragraph{Automated Categorization and Entity Extraction}  
To ensure effective information retrieval, we employed GPT-4o for automated categorization, segmenting each document into key synthesis components: raw materials (\(\mathbf{Y_M}\)), synthesis equipment (\(\mathbf{Y_E}\)), synthesis procedures (\(\mathbf{Y_P}\)), and characterization methods (\(\mathbf{Y_C}\)). Additionally, named entity recognition (NER) was used to identify chemical compounds, equipment, and experimental parameters, improving retrieval accuracy. We applied a confidence-based filtering mechanism, discarding extracted entities with low model confidence scores to enhance precision.

\paragraph{Key Information Segmentation}  
For each of the 17,667 articles confirmed to include a synthesis recipe, we extracted five critical components, denoted as \textbf{X}, \(\mathbf{Y_M}\), \(\mathbf{Y_E}\), \(\mathbf{Y_P}\), and \(\mathbf{Y_C}\). These components capture the end-to-end workflow of materials synthesis, ensuring a structured representation of key experimental details.

\begin{enumerate}
    \item \textbf{X: Target Material, Synthesis Method, and Application Domain}
    
    A concise summary describing:
    \begin{itemize}
        \item \textit{What is being synthesized?} (e.g., Ni-rich layered oxides)
        \item \textit{Which process is used?} (e.g., solvothermal, sol-gel)
        \item \textit{What is the main application?} (e.g., electrode for lithium-ion batteries)
    \end{itemize}
    
    \item \(\mathbf{Y_M}\): \textbf{Raw Materials}
    
    A list of raw materials (e.g., reagents, solvents) and any quantitative details (e.g., molar ratios, concentrations, masses).
    
    \item \(\mathbf{Y_E}\): \textbf{Synthesis Equipment}
    
    A catalog of apparatus (e.g., furnace, autoclave, spin coater) essential for the synthesis steps.
    
    \item \(\mathbf{Y_P}\): \textbf{Synthesis Procedure}
    
    A step-by-step protocol detailing how the reagents are combined and processed (e.g., reaction times, temperatures, pH, stirring speeds).
    
    \item \(\mathbf{Y_C}\): \textbf{Characterization Methods and Results}
    
    Techniques (e.g., X-ray diffraction, electron microscopy) and outcomes (e.g., crystal structure, particle size, electrochemical performance) used to evaluate the synthesized material.
\end{enumerate}

These structured components serve as the foundation for subsequent benchmarking tasks, ensuring that synthesis recipes are consistently represented.

\paragraph{Synthesis Step Extraction}  
A key challenge in structuring synthesis recipes is extracting stepwise procedural details while preserving logical coherence. LLM-based parsing prompts were optimized to capture step dependencies and correctly link conditions like temperature, reaction time, and precursor ratios to experimental steps. Furthermore, synthesis steps were normalized to maintain consistency across different papers, reducing ambiguity in procedural descriptions.\\

{\color{red} 데이터셋 수집 파이프라인 내용 좀 줄임,}

\subsection{Data Verification and Quality Assessment}
To ensure the accuracy of our automatically extracted recipes, we manually verified sampled recipes by eight domain experts, at least a master's student majoring in materials science. These experts evaluated:

\begin{itemize}
    \item \textbf{Completeness:} Did the extracted text capture the full scope of the reported recipe (\textbf{X}, \(\mathbf{Y_M}\), \(\mathbf{Y_E}\), \(\mathbf{Y_P}\), and \(\mathbf{Y_C}\))?
    \item \textbf{Correctness:} Were critical details like temperature values or reagent amounts accurately extracted?
    \item \textbf{Coherence:} Did the extracted recipe retain coherence and avoid contradictory information?
\end{itemize}

\input{table/data/human_verification}
Preliminary reviews indicate that the \emph{majority} of extracted data is highly accurate, especially for articles with well-structured experimental sections. 

Completeness was assessed with relatively high agreement, indicating that key synthesis details were well captured. While its score was slightly lower than correctness and coherence due to occasional omissions of finer experimental details, such as precise molar ratios or characterization settings, the extracted recipes still provide a strong foundation for understanding synthesis procedures. In contrast, correctness and coherence, despite receiving high scores, showed greater variability among evaluators. Differences in how minor inconsistencies—such as variations in equipment names or missing characterization details—were weighted contributed to this variation. Some evaluators viewed these as negligible, while others applied stricter criteria, highlighting the need for clearer annotation guidelines. Overall, these results suggest that the extraction process is already highly effective and can be further refined to enhance the level of detail captured.  
However, manual verification alone is not sufficient to ensure consistent performance across diverse synthesis procedures.  
To systematically evaluate how well models can predict and extract synthesis protocols, we introduce a benchmarking framework that quantitatively assesses model performance on end-to-end synthesis prediction.  

With the dataset validated, the next step is to establish a structured evaluation framework.  
In the following section (Section~\ref{sec:benchmark}), we present a benchmark designed to assess NLP models on materials synthesis prediction, covering key tasks such as precursor and equipment inference, procedure generation, and characterization outcome forecasting.  

% \subsection{Literature Retrieval and Filtering}
% We began by compiling a list of 50 keywords that broadly represent research in materials science, ranging from specific compounds (e.g., ``perovskite,'' ``metal--organic framework'') to broader application domains (e.g., ``battery electrode,'' ``catalysis material''). These keywords were used to query the Semantic Scholar API~\cite{semanticscholar2023}. We restricted the collection of articles that include publicly available PDF files to comply with legal and ethical guidelines for text mining. This process yielded a dataset of 28,685 PDF documents spanning various journals and conferences. 

% \subsection{PDF Conversion and Document Categorization}


% \begin{figure*}[!ht]
%     \begin{subfigure}{.55\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{image/data/element_freq_heatmap.png}
%         \caption{The distribution of elements in the target material shown in the periodic table}
%         \label{fig:data-element-distribution}
%     \end{subfigure}
%     \begin{subfigure}{.43\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{image/data/top10process.png}
%         \caption{Distribution of categorized manufacturing methods}
%         \label{fig:data-process-distribution}
%     \end{subfigure}
%     \caption{Data Distribution}
%     \label{fig:main-data-distribution}
% \end{figure*}


% After retrieving the PDFs, we converted each file to Markdown format using the \texttt{PyMuPDFLLM}~\cite{pymupdf4llm2024}. 
% The resulting Markdown files preserve paragraph structures and metadata while remaining flexible for downstream tasks (e.g., classification, named entity recognition).
% Using the processed Markdown files, we employed GPT-4o~\cite{achiam2023gpt} for an automated categorization step, labeling each article according to:

% \begin{itemize}
%     \item \textbf{Presence of a synthesis recipe:} Whether the text explicitly provides a detailed experimental procedure.
%     \item \textbf{Primary material(s):} The main material name, chemical formula, and class studied (e.g., inorganic oxides, polymers).
%     \item \textbf{Process or synthesis route:} The dominant experimental methods (e.g., hydrothermal, solution-based, vapor deposition).
%     \item \textbf{Application domain:} The intended use-case (e.g., battery, catalysis, biomedical).
% \end{itemize}

% Based on these annotations, we identified 17,667 articles (\(\sim62\%\) of the corpus) containing explicit synthesis ``recipes'', making them highly relevant for tasks involving the prediction or generation of experimental protocols.

% \subsection{Recipe Extraction}
% \label{sec:recipe_extraction}

% \subsubsection{Key Information Segmentation}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{image/data/example.png}
%     \caption{An actual example of extracted recipe.}
%     \label{fig:data-example}
% \end{figure*}

% For each of the 17,667 articles confirmed to include a synthesis recipe, we extracted five critical components, denoted as \textbf{X}, \(\mathbf{Y_M}\), \(\mathbf{Y_E}\), \(\mathbf{Y_P}\), and \(\mathbf{Y_C}\). These components capture the end-to-end workflow of materials synthesis:

% \begin{enumerate}
%     \item \textbf{X: Target Material, Synthesis Method, and Application Domain}
    
%     A concise summary describing:
%     \begin{itemize}
%         \item \textit{What is being synthesized?} (e.g., Ni-rich layered oxides)
%         \item \textit{Which process is used?} (e.g., solvothermal, sol-gel)
%         \item \textit{What is the main application?} (e.g., electrode for lithium-ion batteries)
%     \end{itemize}
    
%     \item \(\mathbf{Y_M}\): \textbf{Raw Materials}
    
%     A list of raw materials (e.g., reagents, solvents) and any quantitative details (e.g., molar ratios, concentrations, masses).
    
%     \item \(\mathbf{Y_E}\): \textbf{Synthesis Equipment}
    
%     A catalog of apparatus (e.g., furnace, autoclave, spin coater) essential for the synthesis steps.
    
%     \item \(\mathbf{Y_P}\): \textbf{Synthesis Procedure}
    
%     A step-by-step protocol detailing how the reagents are combined and processed (e.g., reaction times, temperatures, pH, stirring speeds).
    
%     \item \(\mathbf{Y_C}\): \textbf{Characterization Methods and Results}
    
%     Techniques (e.g., X-ray diffraction, electron microscopy) and outcomes (e.g., crystal structure, particle size, electrochemical performance) used to evaluate the synthesized material.
% \end{enumerate}

% \subsubsection{LLM-Driven Parsing and Annotation}
% The extraction of these elements from each Markdown file was again performed via GPT-4o. We minimized human labor in large-scale annotation by carefully prompting the model to identify and extract relevant text blocks.
% Detailed prompts are described in Appendix~\ref{sec:appendix_annotation}.

% {\color{red}Comprehensive metrics on precision and recall will be added once the manual verification is complete}% 
% Insert final statistics later.




==> old-0213/04_benchmark.tex <==
\section{Benchmark Definition and Tasks}
\label{sec:benchmark}

This section introduces our benchmark for evaluating models on materials synthesis prediction. We outline the task definitions, dataset splits, and evaluation metrics, culminating in a framework reflecting real-world materials science challenges.

\subsection{Task Definition}
The benchmark is designed to simulate end-to-end materials synthesis workflows. Given only the input \textbf{X}—which includes the target material, synthesis method, and application domain—the model must predict all subsequent components:  
\begin{itemize}
    \item \(\mathbf{P_M}\): Raw materials (e.g., reagents, solvents) and their quantities.
    \item \(\mathbf{P_E}\): Required equipment (e.g., furnace, autoclave).
    \item \(\mathbf{P_P}\): Synthesis procedures (e.g., reaction steps, times, temperatures).
    \item \(\mathbf{P_C}\): Characterization methods and expected outcomes.
\end{itemize}

The predicted outputs are compared against ground-truth recipes (\(\mathbf{Y_M}\), \(\mathbf{Y_E}\), \(\mathbf{Y_P}\), and \(\mathbf{Y_C}\)). Evaluations are conducted by either domain experts or an LLM Judge, as detailed in Section~\ref{subsec:metric}. This setup mirrors real-world scenarios where researchers must infer complete synthesis workflows from minimal initial information.

\subsection{Dataset Splits and Distribution}
Our dataset comprises 17,667 articles curated from diverse materials science literature. To ensure robust evaluation, we divide the dataset into three splits based on publication year and journal impact factor (IF):
\begin{itemize}
    \item \textbf{Training Set:} 16,026 articles published before 2024.
    \item \textbf{Test - Standard Impact:} 1,472 articles published in 2024 or later with IF $<$ 10.
    \item \textbf{Test - High Impact:} 169 articles published in 2024 or later with IF $\geq$ 10.
\end{itemize}

The temporal split ensures test data represents unseen future research trends, mitigating data contamination. Further stratification by IF allows targeted assessment of model performance on high-impact research, often involving novel and complex synthesis techniques. This split design evaluates both generalizability and the ability to meet the rigorous standards of top-tier journals.


\subsection{Evaluation Metrics: LLM-as-a-Judge}
\label{subsec:metric}

Evaluating synthesis predictions requires nuanced judgment across multiple dimensions. While human experts provide the gold standard for evaluation, their involvement is time-intensive and costly. To address this, we employ a large language model (LLM) as an efficient alternative evaluator.

\input{table/benchmark/criteria}
\paragraph*{Evaluation Criteria}
Table~\ref{tab:judgment_criteria} outlines the seven criteria for evaluating synthesis recipes.
Each criterion is scored on a 1–5 scale. The overall score is computed as an average across all criteria to reflect recipe quality comprehensively.

\paragraph*{LLM Evaluation Methodology}
We prompted LLMs to generate Chain-of-Thought (CoT) reasoning~\cite{wei2022chain}, followed by structured outputs in JSON format for scoring each criterion. This approach ensures transparency and interpretability in LLM judgments. Detailed prompts and examples are provided in Appendix~\ref{subsec:appendix_llm_judge}.

The reliability of LLM-based evaluations was validated by comparing them against human expert scores. A Pearson correlation coefficient of 0.52 between human and LLM evaluations demonstrates significant alignment, supporting using LLMs as scalable proxies for expert judgment. Further analysis of LLM-human agreement is discussed in Section~\ref{sec:reliability}.

\subsection{Summary and Outlook}
Our benchmark bridges the gap between controlled academic experiments on small datasets and real-world materials synthesis scenarios encountered in laboratories. By encompassing tasks that span precursor selection to characterization prediction, this framework provides a holistic evaluation platform for NLP models. Including high-impact test data ensures relevance to cutting-edge research, while leveraging LLMs as evaluators enable scalable benchmarking without sacrificing rigor.

Future iterations of this benchmark could further incorporate multimodal data (e.g., figures, tables) to enhance its applicability to practical materials science challenges.

==> old-0213/05_llm_judge.tex <==
\section{LLM as a Judge}
\label{sec:reliability}

Ensuring the reliability of the LLM-as-a-Judge framework is critical for establishing trustworthy benchmarking. This section evaluates the alignment between LLM-based judgments and human expert evaluations, analyzing inter-rater agreement across multiple dimensions.

\subsection{Human Expert Evaluation Setup}
\label{subsec:humaneval-setup}

To validate the performance of LLMs as evaluators, we conducted a systematic comparison with domain experts. Below, we outline the evaluation setup:

\paragraph*{Domain Experts}
We enlisted six materials science experts, all holding at least a master's degree and extensive materials synthesis experience. Each expert independently evaluated predictions generated by LLMs using a 1–5 scale across seven criteria, including material appropriateness, procedural coherence, and overall recipe quality (refer to Table~\ref{tab:judgment_criteria}). On average, each evaluation required 23 minutes (\(\sigma=7.57\)) per recipe. Appendix~\ref{sec:appendix_annotation} provides detailed evaluation guidelines and training materials.

To ensure high-quality evaluations, we requested expert confidence scores for each assessment. Three experts with lower confidence scores were excluded from further analysis, leaving three highly confident evaluators whose consensus was used as the ground truth for comparison.

\paragraph*{Dataset}
We selected ten papers from \oursdatashort~that were representative of diverse materials synthesis workflows. Two LLMs (GPT-4o-mini and o1-mini) were tasked with generating recipes (\(\mathbf{P_M}\), \(\mathbf{P_E}\), \(\mathbf{P_P}\), and \(\mathbf{P_C}\)) for each paper based on input \textbf{X}. This resulted in a total of 20 predictions (10 per model). The expert panel evaluated these predictions against ground-truth recipes from the original papers.

\paragraph*{Judge LLMs}
We evaluated four state-of-the-art LLMs as judges:
\begin{itemize}
    \item \textbf{GPT-4o Aug and Nov}: The August and November 2024 release of GPT-4o with enhanced general-purpose capabilities.
    \item \textbf{GPT-4o-mini}: A lightweight version of GPT-4o optimized for efficiency.
    \item \textbf{o1-mini and o3-mini}: Reasoning-based flagship models outperforming in math, code, and academic tasks. We set \texttt{reasoning\_effort = high} for o3-mini.
\end{itemize}

The primary objective was to determine whether these LLMs could reliably approximate human expert evaluations when scoring recipes generated by other models.

\paragraph*{Evaluation Metrics}
We employed the following statistical metrics to measure the alignment between human expert scores and LLM-based judgments:
\begin{itemize}
    \item \textbf{Intraclass Correlation Coefficient (ICC)}: Used to assess consistency among evaluators across all criteria.
    \item \textbf{Pearson Correlation Coefficient}: Measures linear agreement between human and LLM scores.
    \item \textbf{Spearman’s Rank Correlation}: Evaluates rank-order agreement to account for non-linear relationships.
\end{itemize}

High agreement across these metrics would indicate that the LLM Judge can be a reliable proxy for expert evaluations, enabling scalable benchmarking without compromising scientific rigor.


\subsection{Inter-Experts Agreement Analysis}
\input{table/experts/inter-raters-agreement}

To quantify consensus among human evaluators, we computed ICC using a two-way mixed-effects model (ICC3k) for absolute agreement. The inter-expert agreement analysis (Table~\ref{tab:inter-raters}) shows that domain experts exhibit substantial consensus across key evaluation criteria. Specifically, high ICC3k values for \textbf{Procedure Feasibility} (0.70) and \textbf{Overall Score} (0.75) confirm that experts consistently assess the practical executability and overall quality of synthesis recipes. While lower ICC values for \textbf{Procedure Similarity} (0.34) suggest some subjectivity in interpreting "closeness" to ground truth, the overall agreement supports the reliability of expert judgments as a gold standard for evaluation.  


\subsection{LLM-Expert Agreement Analysis}

\input{table/experts/llm-experts-agreement}

The LLM-Expert agreement analysis (Table~\ref{tab:llm-expert}) highlights the viability of using GPT-4o Aug as an automated evaluator. GPT-4o Aug achieves a Pearson correlation of 0.52 with human scores, indicating a strong alignment with expert consensus. 
% Notably, GPT-4o Nov improves this alignment further, achieving a state-of-the-art Pearson correlation of 0.52, demonstrating its ability to approximate expert-level evaluations effectively. 
These results validate utilizing LLMs as cost-effective and scalable alternatives to complete human annotation, particularly for large-scale benchmarking tasks where manual evaluation is impractical.  

\subsection{Summary and Implications}  
\label{subsec:summary_implications}  

The results presented in this section demonstrate the reliability of both human expert evaluations and the LLM Judge within our benchmarking framework. Robust inter-expert agreement and high LLM-expert alignment establish a strong foundation for our evaluation framework. The demonstrated reliability of GPT-4o as a judge supports its integration into our benchmark while maintaining scientific rigor. By leveraging LLM-based evaluation, we achieve significant efficiency gains without compromising the validity or quality of recipe assessments.


==> old-0213/07_con.tex <==
\section{Discussion and Conclusion}
\label{sec:conclusion}

\subsection{Insights from Model Performance}
The experimental results reveal several key insights into the performance of reasoning-based models (o1-mini, o3-mini) compared to general-purpose models (GPT-4o variants) in the context of materials synthesis prediction. While o1-mini and o3-mini excel in tasks requiring structured reasoning, such as mathematics or programming, their performance on the High Impact test set for materials synthesis does not consistently surpass that of GPT-4o Nov. This discrepancy highlights the importance of domain-specific experience and contextual understanding, which GPT-4o Nov appears to capture better.

Materials synthesis involves nuanced decision-making, often relying on implicit knowledge derived from extensive literature exposure and experimental heuristics. The reasoning-centric architecture of o1-mini and o3-mini may lack the contextual flexibility required to adapt to such domain-specific challenges. In contrast, GPT-4o Nov's broader training and enhanced tuning for materials science seem to enable it to generalize more effectively across diverse synthesis scenarios.

\subsection{Effectiveness of Retrieval-Augmented Generation}
The results from the RAG experiments (Figure~\ref{fig:rag_high_impact}) underscore the critical role of retrieval in improving recipe generation quality. By incorporating relevant references from the training set, models can ground their predictions in concrete examples, enhancing both coherence and plausibility. Notably:
\begin{itemize}
    \item Performance gains are most pronounced when \(K \leq 10\), suggesting that a moderate number of high-quality references suffices to provide meaningful context without overwhelming the model.
    \item The retrieval mechanism mainly benefits smaller models like GPT-4o-mini, which cannot independently generate high-quality outputs but can leverage external knowledge effectively.
\end{itemize}

These findings emphasize that retrieval augmentation is not merely a complementary enhancement but a foundational component for advancing synthesis prediction tasks. It bridges gaps in model knowledge by providing domain-relevant examples, thereby mitigating limitations inherent in even state-of-the-art LLMs.

\subsection{Implications and Future Directions}
The observed trends have several implications for future research:
\begin{enumerate}
    \item \textbf{Balancing Reasoning and Contextual Adaptability}: While reasoning-based models like o1-mini and o3-mini excel in structured problem-solving, their application in domains requiring experiential knowledge remains limited. Future architectures should aim to integrate robust reasoning capabilities with mechanisms for capturing domain-specific heuristics.
    
    \item \textbf{Optimizing Retrieval Strategies}: The effectiveness of RAG highlights the need for further exploration of retrieval strategies. Key directions include:
        \begin{itemize}
            \item Developing adaptive retrieval mechanisms that dynamically select the most relevant references based on task complexity.
            \item Investigating multimodal retrieval approaches that incorporate not only text but also figures, tables, and experimental diagrams commonly found in materials science literature.
        \end{itemize}
    
    \item \textbf{Domain-Specific Fine-Tuning}: While GPT-4o Nov demonstrates strong performance, its reliance on general-purpose training data may limit its potential in highly specialized domains. Fine-tuning on curated materials science datasets or integrating expert feedback loops could further enhance its contextual understanding.

    \item \textbf{Human-AI Collaboration}: The nuanced nature of materials synthesis underscores the value of hybrid workflows where LLMs assist human experts by generating candidate recipes or identifying overlooked correlations. Future benchmarks should evaluate standalone model performance and their utility in collaborative settings.
\end{enumerate}

\subsection{Broader Impacts}
The findings from this study extend beyond materials synthesis to other domains where experiential knowledge plays a critical role. By demonstrating the interplay between reasoning capabilities and contextual adaptability, this work provides a roadmap for designing next-generation AI systems capable of tackling complex scientific challenges. Moreover, the demonstrated effectiveness of retrieval augmentation suggests that grounding AI predictions in domain-specific knowledge will remain a cornerstone of progress in applied machine learning.

In conclusion, while current LLMs exhibit promising capabilities, significant opportunities remain for advancing their adaptability, contextual grounding, and collaborative potential. By addressing these challenges, we can accelerate scientific discovery across diverse fields.


==> old-0214/01_intro.tex <==
\section{Introduction}
\label{sec:intro}

Materials synthesis is a cornerstone of scientific progress, driving innovations across various domains such as energy storage, catalysis, electronics, and biomedical devices~\cite{olivetti2020data}. Despite notable advancements, the synthesis process remains empirical, relying on trial-and-error approaches guided by expert intuition~\cite{merchant2023scaling}. This reliance on heuristic methods often impedes novel materials' rapid discovery and optimization. Consequently, a systematic understanding and predictive capability in materials synthesis are critical for accelerating research and development~\cite{huang2023application}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{image/intro/intro_v01_simple.png}
    \caption{An illustrated example of materials synthesis pipeline in \oursbench.}
    \label{fig:intro}
\end{figure}

% In recent years, progress in natural language processing (NLP) has demonstrated promising avenues for extracting actionable insights from unstructured scientific literature. By leveraging large-scale text data, NLP-based methods can help automate the identification of synthesis parameters, uncover hidden correlations, and generate testable hypotheses for materials discovery~\cite{song2023matsci,dunn2020benchmarking}. However, the application of NLP in materials science remains limited by data quality and domain diversity.
% Existing datasets and benchmarks are 1) often small in scale. 2) are prone to noise 3) are narrowly focused target materials~\cite{sun2025critical}. These limitations undermine the generalizability of machine learning models developed for synthesis prediction.

In recent years, Machine Learning (ML) and Large Language Models (LLMs) have emerged as promising tools for leveraging the vast amount of unstructured scientific literature available in materials science. These methods can automate the extraction of synthesis parameters, uncover hidden correlations, and generate testable hypotheses~\cite{song2023matsci,dunn2020benchmarking}. However, several challenges hinder the practical application in this domain: \textbf{1) Data Limitations:} Existing datasets are prone to narrowly focused on specific synthesis procedures~(\eg, solid-state, sol-gel, and solution-based) and prone to noisy~\cite{sun2025critical}, limiting the generalizability of ML models.
\textbf{2) Lack of Standardized Benchmarks:} The absence of comprehensive benchmarks for evaluating end-to-end synthesis prediction models impedes progress and prevents meaningful comparisons across approaches.
\textbf{3) Unclear Model Capabilities:} The current level of performance achievable by ML or LLM models in predicting synthesis workflows remains underexplored.
\textbf{4) Evaluation Challenges:} Determining whether LLMs can reliably approximate human-level evaluations for synthesis predictions is an open question.

To address these challenges, we propose \oursdatalong~(\oursdatashort), a dataset of high-quality 17K material synthesis recipes curated from a large corpus of scientific literature using automated methods. 
Based on this dataset, we designed \oursbench~to benchmark models on tasks that mirror real-world materials synthesis workflows:

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{image/intro/process_v02.png}
    \caption{An illustrated workflow of \oursdatalong~construction.}
    \label{fig:intro_data_collection}
\end{figure}

\begin{enumerate}
    \item \textbf{Predicting raw materials:} Given a target material, models are challenged to generate precursor, solvent, and catalyst identities and predict their respective quantities or ratios.
    \item \textbf{Predicting synthesis equipment:} Models must determine the apparatus for a given synthesis based on the target material and precursor information.
    \item \textbf{Predicting synthesis procedures:} Given the target material, raw materials with proportions, and equipment, the model should generate the procedural steps.
    \item \textbf{Predicting characterization methods and outcomes:} Models must infer the appropriate characterization techniques and their possible outcomes based on complete synthesis details.
\end{enumerate}




Figures~\ref{fig:intro} and~\ref{fig:intro_data_collection} illustrate the overall workflow of our proposed dataset construction and benchmark tasks. By capturing the end-to-end pipeline of materials synthesis, our benchmark provides a holistic framework for evaluating NLP models that can generalize across diverse synthesis methods and materials.

Moreover, we explore the potential of LLMs to act as evaluators for synthesis predictions. While human experts provide the gold standard for evaluation, their involvement is time-intensive and costly. We investigate whether LLMs can reliably approximate human-level judgment across multiple evaluation dimensions. This dual focus—on both model performance and evaluation reliability—aims to advance the integration of data-driven approaches into practical materials science.

In summary, this work makes the following contributions:
\begin{itemize}
    \item We present \oursdatalong~(\oursdatashort), a large-scale dataset of 17K material synthesis recipes curated from the scientific literature~(including the latest literature until 2024).
    \item We introduce \oursbench, a comprehensive benchmark that evaluates models on end-to-end tasks spanning precursor prediction to characterization outcomes.
    \item We assess the capabilities of state-of-the-art LLMs in predicting synthesis workflows and examine their reliability as evaluators compared to human experts.
    \item We provide experimental results highlighting key insights into model performance and propose future directions for improving data-driven approaches in materials science.
\end{itemize}
% By capturing the end-to-end pipeline of materials synthesis, this benchmark lays the groundwork for evaluating and developing NLP models that can effectively generalize across diverse synthesis methods and materials. In particular, our emphasis on real-world workflows provides a holistic perspective that moves beyond isolated prediction tasks to encompass all stages of the synthesis process.

% Ultimately, we aim to facilitate the convergence of data-driven approaches and practical materials science. We strive to spur methodological advancements in NLP and deeper collaborations between the materials science and machine learning communities by offering a rigorous evaluation framework. Through this benchmark, we envision a future where machine-learning models expedite the discovery of novel materials and provide actionable guidance for their synthesis and characterization. 

==> old-0214/02_rel.tex <==
\section{Related Work}

\subsection{Materials Synthesis Datasets}

Several datasets have been developed to support machine learning applications in materials synthesis. Text-mined datasets focus on extracting synthesis procedures from scientific literature using natural language processing (NLP) techniques. For instance, a dataset of 19,488 solid-state synthesis recipes~\cite{kononova2019text} was generated from over 53,000 paragraphs, including details like precursors, operations, and conditions. Similarly, solution-based synthesis datasets~\cite{wang2022dataset} include 35,675 procedures with detailed attributes like precursor quantities and reaction formulas. However, these datasets face significant limitations in quality and completeness. A critical review~\cite{sun2025critical} highlighted issues with the ``4 Vs.'' of data science—volume, variety, veracity, and velocity—arguing that many recipes lack essential reproducibility or predictive modeling information. For example, only 28\% of extracted solid-state synthesis paragraphs yielded complete reactions, and one in four compositions had unspecified stoichiometries. These challenges limit the utility of such datasets for guiding novel materials synthesis.


\subsection{LLMs for Materials Science}

Recent advancements in large language models (LLMs) have showcased their potential to accelerate materials discovery, simulation, and evaluation by automating hypothesis generation~\cite{kumbhar2025hypothesisgenerationmaterialsdiscovery}, predicting material properties~\cite{chiang2024llamplargelanguagemodel}, and even serving as evaluators~\cite{mishra2024llamat}. These systems integrate domain-specific knowledge with computational workflows, offering promising tools for designing novel materials or extracting structured insights from the literature. However, their effectiveness remains constrained by challenges such as limited domain-specific datasets, the need for fine-tuning to handle complex synthesis workflows, and insufficient interpretability in critical decision-making processes. These limitations underscore the need for standardized benchmarks and high-quality datasets to evaluate LLM capabilities in materials science rigorously. Our work addresses these gaps by introducing a comprehensive dataset and benchmark tailored to real-world synthesis workflows while also exploring the reliability of LLMs as evaluators against human experts.


\subsection{LLM-Based Evaluation in Materials Science}

Large Language Models (LLMs) have recently gained attention for their potential to evaluate and predict materials synthesis pathways. Studies demonstrate that fine-tuned LLMs can perform comparable or superior to traditional machine learning models in tasks like precursor selection and synthesizability prediction~\cite{lei2024materials,kim2024large}. For example, LLMatDesign~\cite{jia2024llmatdesign} uses LLMs to design materials by iteratively generating hypotheses and evaluating outcomes autonomously. Benchmarks like ALDbench~\cite{yanguas2024benchmarking} assess LLMs' ability to answer domain-specific questions about atomic layer deposition processes. 

Despite these advancements, using LLMs for evaluating materials synthesis quality remains underexplored. \citeauthor{luo2024large} have investigated human-LLM agreement in other scientific domains, showing promising correlations between LLM predictions and expert evaluations. However, in materials science specifically, systematic experiments comparing LLM-based evaluations with human experts are limited. This gap underscores the need for further research into leveraging LLMs as reliable evaluators in this domain while ensuring alignment with expert judgment.


==> old-0214/03_dataset.tex <==
\section{Data Collection and Preparation}
\label{sec:data_collection}

\subsection{Motivation}
\label{subsec:motivation}

Prior attempts to extract synthesis procedures from materials science literature~\cite{kononova2019text,wang2022dataset} suffer from three critical limitations. First, keyword-based and Word2Vec-driven~\cite{mikolov2013efficient} methods introduce excessive noise, making over \textbf{92\%} of \citeauthor{kononova2019text} and \textbf{98\%} of \citeauthor{wang2022dataset} lack necessary synthesis parameters (e.g., heating temperature, duration, mixing conditions). This issue is particularly severe in solution-based synthesis, where multi-step dependencies lead to incomplete extractions. Second, existing datasets are constrained to a few synthesis techniques (solid-state, solution-based, sol-gel), limiting generalizability. Third, commercial journal restrictions prevent dataset sharing, impeding open-access research.

To address these challenges, we introduce three key innovations:  
1) LLM-driven parsing with GPT-4o for high-accuracy extraction,  
2) A broad synthesis method collection covering ten synthesis techniques,  
3) Exclusive use of open-access sources, ensuring legal dataset distribution.  

\subsection{Collection and Extraction}
\label{subsec:collection_extraction}

Our pipeline retrieves 28,685 open-access articles from the 400K searched articles using the Semantic Scholar API~\cite{semanticscholar2023}, employing 50 expert-selected domain-specific search terms (e.g., “sol-gel synthesis”, “thin film deposition”). PDFs are converted into structured Markdown using \texttt{PyMuPDFLLM}~\cite{pymupdf4llm2024}, preserving paragraph structures and metadata.

We employ GPT-4o~\cite{achiam2023gpt} for multi-stage annotation:
\begin{itemize}
    \item Document categorization: Identifies articles with synthesis procedures and classifies them by material type, synthesis route, and application domain.
    \item Recipe segmentation: Extracts five critical components from each identified article:
    \begin{enumerate}
        \item \textbf{X}: Target material, synthesis method, and application summary.
        \item \(\mathbf{Y_M}\): Raw materials with quantitative details.
        \item \(\mathbf{Y_E}\): Equipment specifications.
        \item \(\mathbf{Y_P}\): Step-by-step procedures.
        \item \(\mathbf{Y_C}\): Characterization methods/results.
    \end{enumerate}
\end{itemize}

Figure~\ref{fig:data-example} presents an example of an extracted synthesis recipe.

\begin{figure*}[!ht]
    \begin{subfigure}{.55\textwidth}
        \centering
        \includegraphics[width=\linewidth]{image/data/element_freq_heatmap.png}
        \caption{Distribution of synthesized elements in the dataset}
        \label{fig:data-element-distribution}
    \end{subfigure}
    \begin{subfigure}{.43\textwidth}
        \centering
        \includegraphics[width=\linewidth]{image/data/top10process.png}
        \caption{Diversity of synthesis methods covered}
        \label{fig:data-process-distribution}
    \end{subfigure}
    \caption{Dataset composition highlighting broad material and synthesis technique coverage.}
    \label{fig:main-data-distribution}
\end{figure*}

This process yielded 17,667 high-quality recipes (\(\sim\) 62\% yield) across 10 synthesis techniques.

\subsection{Quality Verification}
\label{subsec:quality_verification}

To assess the accuracy of extracted recipes, we conducted a manual review with eight domain experts (materials scientists with at least a master’s degree). Evaluators rated sampled recipes based on:

\begin{itemize}
    \item \textbf{Completeness:} Does the extraction capture all synthesis details (\textbf{X}, \(\mathbf{Y_M}\), \(\mathbf{Y_E}\), \(\mathbf{Y_P}\), \(\mathbf{Y_C}\))?
    \item \textbf{Correctness:} Are critical synthesis parameters (e.g., temperature, reagent amounts) accurately extracted?
    \item \textbf{Coherence:} Is the extracted recipe logically structured and internally consistent?
\end{itemize}

\input{table/data/human_verification}

Preliminary evaluations indicate that the majority of extracted recipes exhibit high accuracy, particularly when the original articles contain well-structured experimental sections. Completeness was slightly lower than correctness and coherence due to occasional omissions in fine details (e.g., exact molar ratios or characterization parameters). The main sources of extraction variability stem from minor inconsistencies in reagent terminology and missing processing conditions. These findings underscore the need for refined annotation guidelines to ensure consistency.

While manual verification provides useful insights, it cannot scale to evaluate large datasets comprehensively. To systematically assess extraction quality at scale, we introduce a benchmarking framework in the following section (Section~\ref{sec:benchmark}), evaluating models on precursor identification, equipment inference, procedure generation, and characterization forecasting.


==> old-0214/04_benchmark.tex <==
\section{AlchemyBench}
\label{sec:benchmark}

This section introduces our benchmark for evaluating models on materials synthesis prediction. We outline the motivation for using LLMs as judges, task definitions, dataset splits, and evaluation metrics, culminating in a framework reflecting real-world materials science challenges.

\subsection{Motivation: Why LLM-as-a-Judge?}
\label{subsec:motivation}
The evaluation of general materials synthesis recipes poses unique challenges that necessitate scalable and efficient solutions:
\begin{itemize}
    \item \textbf{Lack of Existing Benchmarks:} There is no established benchmark for evaluating general materials synthesis recipes nor a standardized framework to assess their quality systematically.
    \item \textbf{Limitations of Traditional Metrics:} Commonly used metrics such as BLEU~\cite{papineni2002bleu} and ROUGE~\cite{lin2004rouge} focus on surface-level lexical similarity but fail to capture the semantic requirements of synthesis recipes. \citeauthor{na2023artificial} et al. utilized the Jaccard score to evaluate the set overlap of synthesis procedures but lacks sensitivity to sequential dependencies critical in procedural texts. Additionally, BERTScore~\cite{zhang2019bertscore} leverages contextual embeddings from pretrained language models to measure semantic similarity beyond token matching, offering a more context-aware evaluation. However, despite its advantages, BERTScore often underperforms in the Materials Synthesis Recipe domain, where the intricate sequential dependencies and specialized domain semantics are not fully captured.
    \item \textbf{Cost and Inefficiency of Human Evaluation:} Employing domain experts for recipe evaluation is prohibitively expensive and time-consuming, with an average evaluation time of 23 minutes per recipe ($\sigma=7.57$) in our experiment.
    \item \textbf{Need for Scalable Solutions:} A scalable and high-performance evaluation tool is essential to support high-throughput benchmarking. LLMs offer a promising alternative by providing consistent and interpretable evaluations at scale~\cite{gu2025surveyllmasajudge}.
\end{itemize}

By addressing these challenges, LLM-as-a-Judge enables efficient benchmarking while maintaining alignment with expert evaluations.


\subsection{Task Definition}
\label{subsec:task_definition}
The proposed benchmark simulates end-to-end workflows in materials synthesis. Given an input $\mathbf{X}$ — comprising the target material, synthesis method, and application domain — the model must predict the following components:
\begin{itemize}
    \item $\mathbf{P_M}$: Raw materials (e.g., reagents, solvents) and their quantities.
    \item $\mathbf{P_E}$: Required equipment (e.g., furnace, autoclave).
    \item $\mathbf{P_P}$: Synthesis procedures (e.g., reaction steps, times, temperatures).
    \item $\mathbf{P_C}$: Characterization methods and expected outcomes.
\end{itemize}

The predictions $\mathbf{P_X}=\{\mathbf{P_M,P_E,P_P,P_C}\}$ are compared against ground-truth recipes $\mathbf{Y_X}=\{\mathbf{Y_M}, \mathbf{Y_E}, \mathbf{Y_P}, \mathbf{Y_C}\}$ using the LLM-as-a-Judge framework. The evaluation criteria include appropriateness, completeness, feasibility, and similarity to ground truth. This task setup was designed in collaboration with domain experts and mirrors real-world scenarios where researchers infer complete workflows from minimal initial information.

The LLM-as-a-Judge's overall score $\text{Score}(P_X,Y_X)$ is calculated as follows:
\[
\text{Score}(P_X, P_Y) = \frac{\sum_{i=1}^{N_C} C_i}{N_C}
\]
where $C_i$ represents the score for criterion $i$, and $N_C$ is the total number of criteria. We will introduce the detailed prompt and criteria in Section~\ref{sec:reliability}.

\subsection{Dataset Splits and Distribution}
Our dataset comprises 17,667 articles curated from diverse materials science literature. To ensure robust evaluation, we divide the dataset into three splits based on publication year and journal Impact Factor (IF):
\begin{itemize}
    \item \textbf{Training Set:} 16,026 articles published before 2024.
    \item \textbf{Test - Standard Impact:} 1,472 articles published in 2024 or later with IF $<$ 10.
    \item \textbf{Test - High Impact:} 169 articles published in 2024 or later with IF $\geq$ 10.
\end{itemize}

The temporal split ensures test data represents unseen future research trends, mitigating data contamination. Further stratification by IF allows targeted assessment of model performance on high-impact research, often involving novel and complex synthesis techniques. This split design evaluates both generalizability and the ability to meet the rigorous standards of top-tier journals.




==> old-0214/05_llm_judge.tex <==
\section{LLM as a Judge}
\label{sec:reliability}

Ensuring the reliability of the LLM-as-a-Judge framework is critical for establishing trustworthy benchmarking. This section evaluates the alignment between LLM-based judgments and human expert evaluations, providing a detailed analysis of inter-rater agreement and the statistical metrics used to validate the framework.

\subsection{Evaluation Metrics}
\label{subsec:evaluation_metrics}
\input{table/benchmark/criteria}

Evaluating synthesis recipes requires systematical judgment across multiple dimensions, including material appropriateness, procedural feasibility, etc. We employ three complementary statistical metrics to ensure rigorous assessment: Intraclass Correlation Coefficient (ICC), Pearson Correlation Coefficient, and Spearman’s Rank Correlation.

The \textbf{ICC} is used to measure inter-rater reliability, capturing the consistency of scores across evaluators. This metric is particularly relevant for subjective judgment tasks, where expert agreement is a gold standard for evaluation reliability. The \textbf{Pearson Correlation Coefficient} quantifies the linear alignment between human and LLM scores, providing insight into how closely LLM judgments approximate expert evaluations on a continuous scale. 
% Finally, the \textbf{Spearman’s Rank Correlation} evaluates rank-order agreement, making it suitable for scenarios where relative ranking of recipe quality is more important than absolute scores.

By combining these metrics, we ensure a comprehensive evaluation that captures both consistency and alignment across multiple dimensions. This approach addresses limitations in traditional metrics such as BLEU and ROUGE-L, which focus on surface-level text similarity and fail to account for the contextual appropriateness or procedural coherence required in synthesis recipes.

\subsection{Human Expert Evaluation Setup}
\label{subsec:humaneval_setup}

To establish a reliable ground truth for comparison, we enlisted eight domain experts from three organizations (2/3/3) with extensive experience in materials synthesis. Each expert independently evaluated model-generated recipes based on seven criteria outlined in Table~\ref{tab:judgment_criteria}, scoring each criterion on a 1–5 scale. On average, each evaluation required 23 minutes (\(\sigma=7.57\)) per recipe. To ensure high-quality assessments, we collected expert confidence scores and highlighted the agreement of one organization of three experts with the highest confidence levels on average (denoted as `High').

The dataset used for evaluation consisted of ten representative papers from \oursdatashort~covering diverse synthesis workflows. A professor in the field of materials science selected these papers based on the expertise of evaluators. Prediction recipes were generated by two models (GPT-4o-mini and o1-mini), resulting in 20 predictions evaluated by human experts and LLM judges.

\subsection{Inter-Expert Agreement Analysis}
\label{subsec:inter_rater_analysis}
\input{table/experts/inter-raters-agreement}

We computed the Intraclass Correlation Coefficient (ICC) using a two-way mixed-effects model (ICC3k) to quantify consensus among human evaluators. As shown in Table~\ref{tab:inter-raters}, high ICC values were observed for ``Procedure Feasibility" (0.70) and ``Overall Score" (0.75), indicating substantial agreement among experts on these critical criteria. Lower ICC values for ``Procedure Similarity`` (0.34) reflect inherent subjectivity in assessing how closely predicted procedures match ground truth recipes. However, the overall agreement supports the reliability of expert judgments as a gold standard for evaluation.

\subsection{LLM-Expert Agreement Analysis}
\label{subsec:llm_expert_analysis}
\input{table/experts/llm-experts-agreement}

To evaluate the alignment between LLM-based judgments and human expert evaluations, we analyzed the performance of four state-of-the-art LLMs using Pearson correlation coefficients. 
We set the temperature to zero for GPT-4o and GPT-4o-mini\footnote{o1-mini and o3-mini do not allow to set temperature.}.

Table~\ref{tab:llm-expert} summarizes these results. Notably, GPT-4o Aug achieved a Pearson correlation of 0.80 (\(p=0.00\)), demonstrating statistically a strong positive alignment with expert scores. These results surpass traditional metrics like BLEU (\(-0.16\), \(p=0.50\)) and ROUGE-L (0.06, \(p=0.80\)), which fail to capture expert-level aspects of recipe quality.

The demonstrated alignment between GPT-4o Aug and the high-confidence group validates its use as a scalable proxy for expert judgment in large-scale benchmarking tasks where manual evaluation is impractical.

\subsection{Comparison with Traditional Metrics}
\label{subsec:traditional_metrics}

Traditional metrics such as BLEU, ROUGE-L, and BERTScore were also evaluated as baselines but failed to align with human evaluations meaningfully (Table~\ref{tab:llm-expert}). These metrics rely on surface-level textual similarity and do not account for contextual appropriateness or procedural coherence—key aspects of synthesis recipe quality. In contrast, LLM-based evaluations explicitly incorporate these dimensions through structured scoring criteria (Table~\ref{tab:judgment_criteria}), making them better suited for this task.

\subsection{Summary and Implications}
\label{subsec:summary_implications}

The results presented in this section demonstrate the reliability of both human expert evaluations and LLM-based judgments within our benchmarking framework. High inter-expert agreement establishes the validity of human evaluations as a gold standard. At the same time, significant alignment between GPT-4o Aug and expert scores supports its integration into our benchmark as a scalable alternative to manual annotation.

Our framework achieves robust benchmarking without compromising scientific rigor by leveraging advanced statistical metrics and addressing limitations in traditional evaluation methods. Future work could further enhance alignment by incorporating pairwise comparison techniques or fine-tuning LLMs using reinforcement learning from human feedback.

% \subsection{Human Expert Evaluation Setup}
% \label{subsec:humaneval-setup}
% \input{table/benchmark/criteria}


% To validate the performance of LLMs as evaluators, we conducted a systematic comparison with domain experts. Below, we outline the evaluation setup:

% \paragraph*{Domain Experts}
% We enlisted six materials science experts, all holding at least a master's degree and extensive materials synthesis experience. Each expert independently evaluated predictions generated by LLMs using a 1–5 scale across seven criteria, including material appropriateness, procedural coherence, and overall recipe quality (refer to Table~\ref{tab:judgment_criteria}). On average, each evaluation required 23 minutes (\(\sigma=7.57\)) per recipe. Appendix~\ref{sec:appendix_annotation} provides detailed evaluation guidelines and training materials.

% To ensure high-quality evaluations, we requested expert confidence scores for each assessment. Three experts with lower confidence scores were excluded from further analysis, leaving three highly confident evaluators whose consensus was used as the ground truth for comparison.

% \paragraph*{Dataset}
% We selected ten papers from \oursdatashort~that were representative of diverse materials synthesis workflows. Two LLMs (GPT-4o-mini and o1-mini) were tasked with generating recipes (\(\mathbf{P_M}\), \(\mathbf{P_E}\), \(\mathbf{P_P}\), and \(\mathbf{P_C}\)) for each paper based on input \textbf{X}. This resulted in a total of 20 predictions (10 per model). The expert panel evaluated these predictions against ground-truth recipes from the original papers.

% \paragraph*{Judge LLMs}
% We evaluated five state-of-the-art LLMs as judges:
% \begin{itemize}
%     \item \textbf{GPT-4o Aug and Nov}: The August and November 2024 release of GPT-4o with enhanced general-purpose capabilities.
%     \item \textbf{GPT-4o-mini}: A lightweight version of GPT-4o optimized for efficiency.
%     \item \textbf{o1-mini and o3-mini}: Reasoning-based flagship models outperforming in math, code, and academic tasks.
% \end{itemize}

% The primary objective was to determine whether these LLMs could reliably approximate human expert evaluations when scoring recipes generated by other models. We set reasoning\_effort to high for o3-mini, set temperature to zero for GPT-4o and GPT-4o-mini\footnote{o1-mini and o3-mini do not allow to set temperature.}.

% \paragraph*{Evaluation Metrics}
% We employed the following statistical metrics to measure the alignment between human expert scores and LLM-based judgments:
% \begin{itemize}
%     \item \textbf{Intraclass Correlation Coefficient (ICC)}: Used to assess consistency among evaluators across all criteria.
%     \item \textbf{Pearson Correlation Coefficient}: Measures linear agreement between human and LLM scores.
%     \item \textbf{Spearman’s Rank Correlation}: Evaluates rank-order agreement to account for non-linear relationships.
% \end{itemize}

% High agreement across these metrics would indicate that the LLM Judge can be a reliable proxy for expert evaluations, enabling scalable benchmarking without compromising scientific rigor.


% \subsection{Inter-Experts Agreement Analysis}
% \input{table/experts/inter-raters-agreement}

% To quantify consensus among human evaluators, we computed ICC using a two-way mixed-effects model (ICC3k) for absolute agreement. The inter-expert agreement analysis (Table~\ref{tab:inter-raters}) shows that domain experts exhibit substantial consensus across key evaluation criteria. Specifically, high ICC3k values for \textbf{Procedure Feasibility} (0.70) and \textbf{Overall Score} (0.75) confirm that experts consistently assess the practical executability and overall quality of synthesis recipes. While lower ICC values for \textbf{Procedure Similarity} (0.34) suggest some subjectivity in interpreting "closeness" to ground truth, the overall agreement supports the reliability of expert judgments as a gold standard for evaluation.  


% \subsection{LLM-Expert Agreement Analysis}

% \input{table/experts/llm-experts-agreement}

% The LLM-Expert agreement analysis (Table~\ref{tab:llm-expert}) highlights the viability of using GPT-4o Aug as an automated evaluator. GPT-4o Aug achieves a Pearson correlation of 0.52 with human scores, indicating a strong alignment with expert consensus. 
% % Notably, GPT-4o Nov improves this alignment further, achieving a state-of-the-art Pearson correlation of 0.52, demonstrating its ability to approximate expert-level evaluations effectively. 
% These results validate utilizing LLMs as cost-effective and scalable alternatives to complete human annotation, particularly for large-scale benchmarking tasks where manual evaluation is impractical.  

% \subsection{Summary and Implications}  
% \label{subsec:summary_implications}  

% The results presented in this section demonstrate the reliability of both human expert evaluations and the LLM Judge within our benchmarking framework. Robust inter-expert agreement and high LLM-expert alignment establish a strong foundation for our evaluation framework. The demonstrated reliability of GPT-4o as a judge supports its integration into our benchmark while maintaining scientific rigor. By leveraging LLM-based evaluation, we achieve significant efficiency gains without compromising the validity or quality of recipe assessments.


==> old-0214/06_exp.tex <==
\section{Experiments}
\label{sec:experiment}

This section evaluates the performance of five LLMs on the proposed benchmark using our LLM-as-a-Judge framework based on GPT-4o Aug. We analyze their performance across multiple metrics, including mean and maximum scores, score distributions, and the impact of retrieval-augmented generation (RAG).

\subsection{Experiment Setup}
\label{subsec:experiment_setup}

To comprehensively evaluate the models, we conducted experiments with the following setup:

\paragraph*{Base LLMs}
We evaluated four LLMs, including reasoning-based models (o3-mini) and general-purpose models (GPT-4o variants). The knowledge cutoff of these models is October 2023, minimizing potential data contamination in our test sets\footnote{The knowledge cutoff of OpenAI's models is described in \url{https://platform.openai.com/docs/models}.}. Moreover, we varied the reasoning\_effort of o3-mini to ensure the effectiveness of reasoning length in materials synthesis.

\paragraph*{Evaluation Framework}
Each model generated synthesis recipes for both the \testhi~and \testsi. Recipes were evaluated using our LLM-as-a-Judge method based on GPT-4o Aug. The evaluation criteria focused on material appropriateness, procedural feasibility, and overall recipe quality.
\paragraph*{Retrieval-Augmented Generation (RAG)}
To assess the impact of retrieval-augmented generation~\cite{lewis2020retrieval}, we implemented a RAG pipeline using OpenAI Embeddings~\cite{OpenAIEmbeedings2022}, which model is text-embedding-3-large with 3072 dimensions. For each input \(X\), we retrieved the top-\(K\) most similar contributions from the training set based on cosine similarity in embedding space and their recipes. These retrieved recipes were included as references in the prompts provided to the LLMs. We evaluated \(K = \{0, 1, 5, 10, 25\}\) to study how increasing contextual information affects recipe generation quality.

This experimental setup ensures a thorough evaluation of both baseline performance and improvements achieved through retrieval augmentation. Due to computational constraints, RAG experiments were conducted on three representative models (GPT-4o Nov, GPT-4o-mini, and o3-mini) using only the \testhi.

\subsection{Insights from Experimental Results}
\label{subsec:insights}


The experimental results provide valuable insights into the challenges and opportunities in materials synthesis prediction, structured around the following research questions:


\input{table/exp/base_results}
\paragraph*{RQ1: Is High-Impact Set More Challenging than Standard-Impact Set?}
The results confirm that \testhi~is indeed more challenging than \testsi. Across all models, average scores on the \testhi~were generally lower than those on the \testsi. For example, o3-mini-high achieved an average score of \(3.759 \pm 0.407\) on \testhi~compared to \(3.885 \pm 0.377\) on \testsi~(Table~5). This discrepancy highlights the increased complexity of High-Impact synthesis workflows, which often involve novel materials or cutting-edge techniques requiring greater reasoning and contextual understanding.

\paragraph*{RQ2: Are Reasoning-Based Models Effective in Materials Science?}
The reasoning-based models, particularly o3-mini-high, demonstrated superior performance compared to general-purpose models like GPT-4o Nov. On both High-Impact and Standard-Impact datasets, o3-mini-high consistently achieved higher mean scores and broader score distributions, indicating its ability to generate high-quality recipes in complex scenarios. For instance, o3-mini-high achieved a maximum score of \(4.71\) on High-Impact, matching GPT-4o Nov but with a higher average score (\(3.759\) vs. \(3.709\)).

These results align with trends observed in domains such as mathematics and programming, where reasoning-based models excel due to their structured problem-solving capabilities. However, the performance gap between o3-mini-high and other reasoning-based variants (e.g., o3-mini-medium) suggests that high reasoning capabilities are essential for tackling the nuanced challenges of materials science.

\paragraph*{RQ3: Does RAG Improve Performance?}
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{image/exp/rag_high_impact.png}
    \caption{Impact of the Retrieval Augmented Generation (RAG) in \testhi.}
    \label{fig:rag_high_impact}
\end{figure}
The experimental results confirm that RAG significantly enhances model performance by grounding predictions in domain-relevant examples retrieved from the training set. As shown in Figure~\ref{fig:rag_high_impact}, increasing \(K\) (the number of retrieved references) improves overall scores for all tested models, with notable differences in how reasoning-based and general-purpose models benefit from retrieval.

For o3-mini (high), performance diminish beyond \(K=5\), achieving a maximum score of \(4.0\) at \(K=5\). This suggests that while retrieval provides valuable context, these models already possess strong reasoning capabilities to generate high-quality recipes independently.

In contrast, \textbf{GPT-4o Nov}, a general-purpose model, exhibits consistent improvement even beyond \(K=5\), ultimately achieving a competitive overall score of \(3.98\) at \(K=25\). This result highlights that retrieval mechanisms can partially compensate for the lack of inherent reasoning capabilities in general-purpose models by providing explicit contextual information. The marginal difference between GPT-4o Nov (\(3.98\)) and o3-mini-high (\(4.0\)) suggests that retrieval can narrow the performance gap between reasoning-based and general-purpose models in materials science tasks.

These findings underscore two key insights:
1) Retrieval augmentation is a foundational component for improving recipe generation quality, particularly for general-purpose models that rely heavily on external context.
2) The retrieval effectiveness depends on the model architecture and the quality of the training set. The observed gains validate the utility of our curated dataset as a reliable source of domain-specific knowledge.

However, diminishing returns beyond \(K=5\) for most models suggest an optimal range for reference incorporation, balancing contextual relevance with cognitive load on the model.

==> old-0214/07_con.tex <==
\section{Conclusion}
\label{sec:conclusion}

This work introduces a comprehensive benchmark for evaluating NLP models in the context of materials synthesis prediction, addressing critical challenges in data-driven materials science. By curating a large-scale dataset and designing tasks that reflect real-world synthesis workflows, we provide a robust framework for assessing model capabilities across precursor selection, equipment inference, procedure generation, and characterization prediction. Our experiments demonstrate the potential of reasoning-based models, such as o3-mini, to excel in structured problem-solving tasks, achieving superior performance compared to general-purpose models like GPT-4o variants. Integrating retrieval-augmented generation (RAG) further enhances recipe quality by grounding predictions in domain-relevant examples, with optimal gains observed up to \(K=10\).

The insights derived from this study highlight the importance of reasoning capabilities and contextual adaptability in advancing materials synthesis prediction. While reasoning-based models outperform general-purpose counterparts in generating coherent and feasible workflows, their application can be further enhanced by leveraging retrieval mechanisms and domain-specific fine-tuning. These findings underscore the need for hybrid approaches that combine robust reasoning architectures with adaptive retrieval strategies to address the nuanced requirements of materials science tasks. This work lays the foundation for interdisciplinary innovation by bridging NLP and materials science, accelerating progress toward data-driven materials discovery and design.


==> prompt/prediction_1shot.tex <==
You are an expert in material science and chemical synthesis. Your task is to design a detailed material synthesis recipe, considering the following **key contributions**:
Your output should follow the exact structure and format of the below example. Provide precise details for each section, including materials, equipment, and step-by-step procedures.

-- Example Input --
## Key Contributions
- **Novel materials or compounds**: Nanoceria-based sorbents for enhanced sorption of low specific activity [99]Mo.
- **Unique synthesis methods**: Development of CeO2 nanoparticles using wet chemical precipitation and hydrothermal approaches.
- **Specific applications or domains**: Potential application in the development of [99]Mo/[99m]Tc generators for nuclear medicine. 
-- Example Output --
## Materials
- **Precursor Materials**:
  - Cerium nitrate hexahydrate (Ce(NO3)3\cdot6H2O): 2g.
  - Sodium hydroxide: 0.4 M solution.
- **Solvents**:
  - Milli-Q water.
  - Ethanol absolute (1:4 v/v with water for chemical precipitation, 4:1 v/v for hydrothermal method).
- **Reagents**:
  - Nitric acid (HNO3).
  - 1 M NaOH solution for adjusting pH.
- **Specifications**:
  - All chemicals of analytical grade from Merck, Darmstadt, Germany.
## Synthesis Equipment
- **Centrifuge**: Used at 4000 rpm for 15 minutes.
- **Drying Oven**: Temperature range of 50–70 $^{\circ}$C for 12 hours.
- **Teflon-lined Stainless Steel Autoclave**: Used for hydrothermal synthesis at 150 $^{\circ}$C for 12 hours.
## Synthesis Procedure
### Wet Chemical Precipitation
1. Dissolve 2 g of Ce(NO3)3\cdot6H2O in a mixture of Milli-Q water and ethanol (1:4 v/v).
2. Add the solution drop-wise to a 0.4 M sodium hydroxide solution under continuous stirring, maintaining pH ~11.
3. Stir until a yellow suspension forms (~30 min). 
4. Wash the precipitate with de-ionized water and ethanol; centrifuge and dry at 50–70 $^{\circ}$C for 12 h. 
5. Denote the sample as CP (Chemical Precipitation).
### Hydrothermal Modification
1. Transfer the precipitated NPs into a Teflon-lined stainless-steel autoclave.
2. Seal and maintain at 150 $^{\circ}$C for 12 hours.
3. Wash, centrifuge, and dry the precipitate at 70 $^{\circ}$C for 12 h.
4. Denote the sample as HT (Hydrothermal Treatment).

-- Prediction Input --
Now, predict the synthesis recipe for the given key contributions:
{contributions}

==> prompt/prediction_1shot_example.tex <==
-- Example Input --
## Key Contributions
- **Novel materials or compounds**: Nanoceria-based sorbents for enhanced sorption of low specific activity [99]Mo.
- **Unique synthesis methods**: Development of CeO2 nanoparticles using wet chemical precipitation and hydrothermal approaches.
- **Specific applications or domains**: Potential application in the development of [99]Mo/[99m]Tc generators for nuclear medicine. 
-- Example Output --
## Materials
- **Precursor Materials**:
  - Cerium nitrate hexahydrate (Ce(NO3)3\cdot6H2O): 2g.
  - Sodium hydroxide: 0.4 M solution.
- **Solvents**:
  - Milli-Q water.
  - Ethanol absolute (1:4 v/v with water for chemical precipitation, 4:1 v/v for hydrothermal method).
- **Reagents**:
  - Nitric acid (HNO3).
  - 1 M NaOH solution for adjusting pH.
- **Specifications**:
  - All chemicals of analytical grade from Merck, Darmstadt, Germany.
## Synthesis Equipment
- **Centrifuge**: Used at 4000 rpm for 15 minutes.
- **Drying Oven**: Temperature range of 50–70 $^{\circ}$C for 12 hours.
- **Teflon-lined Stainless Steel Autoclave**: Used for hydrothermal synthesis at 150 $^{\circ}$C for 12 hours.
## Synthesis Procedure
### Wet Chemical Precipitation
1. Dissolve 2 g of Ce(NO3)3\cdot6H2O in a mixture of Milli-Q water and ethanol (1:4 v/v).
2. Add the solution drop-wise to a 0.4 M sodium hydroxide solution under continuous stirring, maintaining pH ~11.
3. Stir until a yellow suspension forms (~30 min). 
4. Wash the precipitate with de-ionized water and ethanol; centrifuge and dry at 50–70 $^{\circ}$C for 12 h. 
5. Denote the sample as CP (Chemical Precipitation).
### Hydrothermal Modification
1. Transfer the precipitated NPs into a Teflon-lined stainless-steel autoclave.
2. Seal and maintain at 150 $^{\circ}$C for 12 hours.
3. Wash, centrifuge, and dry the precipitate at 70 $^{\circ}$C for 12 h.
4. Denote the sample as HT (Hydrothermal Treatment).
